Evaluating Concurrent Robustness of Language Models Across Diverse Challenge Sets

Language models, characterized by their black-box nature, often hallucinate and display sensitivity to input perturbations, causing concerns about trust. To enhance trust, it is imperative to gain a comprehensive understanding of the model's failure modes and develop effective strategies to improve their performance. In this study, we introduce a methodology designed to examine how input perturbations affect language models across various scales, including pre-trained models and large language models (LLMs). Utilizing fine-tuning, we enhance the model's robustness to input perturbations. Additionally, we investigate whether exposure to one perturbation enhances or diminishes the model's performance with respect to other perturbations. To address robustness against multiple perturbations, we present three distinct fine-tuning strategies. Furthermore, we broaden the scope of our methodology to encompass large language models (LLMs) by leveraging a chain of thought (CoT) prompting approach augmented with exemplars. We employ the Tabular-NLI task to showcase how our proposed strategies adeptly train a robust model, enabling it to address diverse perturbations while maintaining accuracy on the original dataset. https://msin-infotabs.github.io/

==> TableExample.tex <==
% % \begin{table}[!ht]
% % \small
% % \renewcommand{\arraystretch}{1} % Adjust the value as needed
% % \centering
% % \begin{tabularx}{\linewidth}{l X}
% %   \toprule
% %   \multicolumn{2}{c}{\textbf{Case Closed}} \\
% %   \midrule
% %   \textbf{Written by} & Takahiro Arai \\
% %   \textbf{Published by} & Shogakukan \\
% %   \textbf{English publisher} & SG Shogakukan Asia \\
% %   \textbf{Demographic} & Shonen \\
% %   \textbf{Magazine} & Weekly Shonen Sunday \\
% %   \textbf{Original run} & May 9, 2018 - present \\
% %   \textbf{Volumes} & 2 (List of volumes) \\
% %  \bottomrule
% %  \multicolumn{2}{l}{{\textbf{H1}}: 'Case Closed' was written by Takahiro Arai and}\\
% %  \multicolumn{2}{l}{ published by Shogakukan. \textcolor{cadmiumgreen}{(E)}}\\
% %  \multicolumn{2}{l}{{\textbf{H1'}}: 'Case Closed' was writtKen b Takhahiro Arai }\\
% %  \multicolumn{2}{l}{and publihsed by Shogakukn.\textcolor{cadmiumgreen}{(E)}}\\
% %  \hline
% %  \multicolumn{2}{l}{{\textbf{H2}}: 'Case Closed' was a long-running Japanese }\\
% %   \multicolumn{2}{l}{comic serial.\textcolor{cadmiumgreen}{(E)}}\\
% %   \multicolumn{2}{l}{{\textbf{H2'}}: 'Case Closed' was not a long-running Japanese }\\
% %   \multicolumn{2}{l}{comic serial.\textcolor{red}{(C)}}\\
% %   \hline
% %   \multicolumn{2}{l}{{\textbf{H3}}: 'Case Closed' was made into an anime called} \\
% %   \multicolumn{2}{l}{Detective Conan.\textcolor{gray}{(N)}}\\
% %   \multicolumn{2}{l}{{\textbf{H3'}}: Detective Conan was an anime adaptation} \\
% %   \multicolumn{2}{l}{of 'Case Closed'.\textcolor{gray}{(N)}} \\
% %   \hline
% %     \multicolumn{2}{l}{{\textbf{H4}}: 'Case Closed' has been running for more than} \\
% %   \multicolumn{2}{l}{5 years\textcolor{cadmiumgreen}{(E)}}\\
% %   \multicolumn{2}{l}{{\textbf{H4'}}: 'Case Closed' has been running for more than} \\
% %   \multicolumn{2}{l}{10 years\textcolor{red}{(C)}}\\
% %   \hline
% %    \multicolumn{2}{l}{{\textbf{H5}}: 'Case Closed' was published in English by SG } \\
% %   \multicolumn{2}{l}{Shogakukan Asia\textcolor{cadmiumgreen}{(E)}}\\
% %   \multicolumn{2}{l}{{\textbf{H5'}}: 'Case Closed' was published in English by SG} \\
% %     \multicolumn{2}{l}{Shogakukan Australia\textcolor{red}{(C)}}\\
% % \end{tabularx}
% % \caption{\textbf{An example of tabular premise and hypotheses from \parentDatasetName~ \cite{gupta-etal-2020-infotabs}.}
% % Original hypotheses (H1,H2,H3,H4,H5) and perturbed hypothesis \textbf{(H1',H2',H3',H4',H5')} representing character,negation,paraphrasing,numeric and location perturbations respectively. 
% % \\ Labelled as \textcolor{cadmiumgreen}{E}ntailment,\textcolor{red}{C}ontradiction or \textcolor{gray}{N}eutral.
% % \\ 
% % The \textbf{bold} entries, which correspond to the first column, are the keys, while the corresponding entries in the second column of the same row are their respective values.}
% % \label{tab:example}
% % \end{table}


% \begin{table}
% %\begin{center}
% \centering
% \renewcommand{\arraystretch}{1}
% \footnotesize{
% \begin{tabular}{l l}\\
% \hline
% \multicolumn{2}{c}{\textbf{Case Closed}} \\
% \hline
%   \textbf{Written} & Takahiro Arai \\ 
%   \textbf{Publish} & Shogakukan \\
%   \textbf{Eng. Publish} & SG Shogakukan Asia \\
%   \textbf{Demographic} & Shonen \\
%   \textbf{Magazine} & Weekly Shonen Sunday \\
%   \textbf{Orig. Run} & May 9, 2018 - present \\
%   \textbf{Volumes} & 2 (List of volumes) \\
% \hline
% \end{tabular}}
% % \end{subtable}
% %\end{center}
% \begin{tabular}{cc}
% %\centering
% \begin{center}
% \footnotesize 
% {
% \fbox{\begin{minipage}{23.3em}
%     \textbf{H$_1$:} Takahiro Arai wrote `Case Closed' comic series. \textcolor{cadmiumgreen}{(E)} \\
%               % 'Case Closed' was written by Takahiro Arai and published by Shogakukan.  \\
%                \textbf{H$_1^'$:} Takahiro Arai wotte `Case Closed' comci series. \textcolor{cadmiumgreen}{(E)} 
%                % 'Case Closed' was writtKen b Takhahiro Arai and publihsed by Shogakukan.
%                \\
%                % \vspace{-0.7em}
%                % \midrule
%                % \hline
%                % \vspace{0.7em}
%                 \textbf{H$_2$:} `Case Closed' is a long-term comic series.   
%                 % 'Case Closed’ was a long-running Japanese comic serial. 
%                 \textcolor{cadmiumgreen}{(E)} 
%                 \\
%                \textbf{H$_2^'$:}  % 'Case Closed’ was not a long-running Japanese comic serial. 
%                `Case Closed' isn't a long-term comic series.  \textcolor{red}{(C)} \\
%                % \vspace{-0.7em}
%                % \midrule
%                % \hline
%                % \vspace{0.7em}
%                 \textbf{H$_3$:}  % ’Case Closed’ was made into an anime called Detective Conan. 
%                 `Case Closed' became the anime Detective Conan \textcolor{gray}{(N)} \\
%                \textbf{H$_3^'$:}  
%                Detective Conan is `Case Closed' anime version. \textcolor{gray}{(N)} \\
%                % \hline
%                % \vspace{0.7em}
%                % \vspace{-0.7em}
%                % \midrule 
%                 \textbf{H$_4$:}   % ’Case Closed’ has been running for more than 5 years. 
%                 `Case Closed' has run over 5 years.\textcolor{cadmiumgreen}{(E)} \\
%                \textbf{H$_4^'$:}  % ’Case Closed’ has been running for more than 10 years. 
%                `Case Closed' has run over 10 years.\textcolor{red}{(C)} \\ 
%                % \vspace{-0.7em}
%                % \midrule 
%                % \hline
%                % \vspace{0.7em}
%                 \textbf{H$_5$:} Shogakukan Asia published `Case Closed' (Eng).
%                 % ’Case Closed’ was published in English by SG Shogakukan Asia 
%                 \textcolor{cadmiumgreen}{(E)}\\ \textbf{H$_5^'$:}  Shogakukan UK published `Case Closed' (Eng).
%                 % ’Case Closed’ was published in English by SG Shogakukan Australia 
%                 \textcolor{red}{(C)}
% \end{minipage}}} 
% \end{center}
% \end{tabular}
% \vspace{-0.5em}
% \caption{\small{Tabular premise and hypotheses example from \parentDatasetName ~\cite{gupta-etal-2020-infotabs}. Original (H$_1$-H$_5$) and perturbed hypotheses (H$_1^'$-H$_5^'$) represent character, negation, paraphrasing, numeric, and location perturbations. Labeled as \textcolor{cadmiumgreen}{E}, \textcolor{red}{C}, or \textcolor{gray}{N}. \textbf{Bold} entries are keys; adjacent entries are their values.}}
% % \caption{\small \textbf{An example of tabular premise and hypotheses from \parentDatasetName~ \cite{gupta-etal-2020-infotabs}.}
% % Original hypotheses (H1,H2,H3,H4,H5) and perturbed hypothesis \textbf{(H1',H2',H3',H4',H5')} representing character,negation,paraphrasing,numeric and location perturbations respectively.  Labelled as \textcolor{cadmiumgreen}{E}ntailment,\textcolor{red}{C}ontradiction or \textcolor{gray}{N}eutral. The \textbf{bold} entries, which correspond to the first column, are the keys, while the corresponding entries in the second column of the same row are their respective values.} 
% \vspace{-1.75em}
% \label{tab:example}
% \end{table}


% \documentclass{article} % Or your preferred document class
% \usepackage{subfig} % For side-by-side tables
% \usepackage{color}  % For text coloring
% \usepackage{graphicx} % If you need to include any graphics

% Color definitions
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{red}{rgb}{1.0, 0.0, 0.0}
\definecolor{gray}{rgb}{0.5, 0.5, 0.5}

% \begin{document}

\begin{figure} 
\centering 
\begin{subtable}[b]{0.45\textwidth} 
\centering
\renewcommand{\arraystretch}{1}
\footnotesize{
\begin{tabular}{l l}\\
\hline
\multicolumn{2}{c}{\textbf{Case Closed}} \\
\hline
\textbf{Written} & Takahiro Arai \\
\textbf{Publish} & Shogakukan \\
\textbf{Eng. Publish} & SG Shogakukan Asia \\
\textbf{Demographic} & Shonen \\
\textbf{Magazine} & Weekly Shonen Sunday \\
\textbf{Orig. Run} & May 9, 2018 - present \\
\textbf{Volumes} & 2 (List of volumes) \\
\hline
\end{tabular}}
\caption{Case Closed Details} 
\label{tab:case_details}
\end{subtable}
\hfill 
\begin{subtable}[b]{0.45\textwidth}  
\centering
\footnotesize
{
\fbox{\begin{minipage}{25em}
\textbf{H$_1$:} Takahiro Arai wrote `Case Closed' comic series. \textcolor{cadmiumgreen}{(E)} \\
\textbf{H$_1^'$:} Takahiro Arai wotte `Case Closed' comci series. \textcolor{cadmiumgreen}{(E)}
\\
\textbf{H$_2$:} `Case Closed' is a long-term comic series.\textcolor{cadmiumgreen}{(E)}
\\
\textbf{H$_2^'$:}`Case Closed' isn't a long-term comic series.\textcolor{red}{(C)} \\
\textbf{H$_3$:}`Case Closed' became the anime Detective Conan \textcolor{gray}{(N)} \\
\textbf{H$_3^'$:}Detective Conan is `Case Closed' anime version. \textcolor{gray}{(N)} \\
\textbf{H$_4$:}`Case Closed' has run over 5 years.\textcolor{cadmiumgreen}{(E)} \\
\textbf{H$_4^'$:}`Case Closed' has run over 10 years.\textcolor{red}{(C)} \\
\textbf{H$_5$:} Shogakukan Asia published `Case Closed' (Eng). \textcolor{cadmiumgreen}{(E)}\\ 
\textbf{H$_5^'$:}Shogakukan UK published `Case Closed' (Eng). \textcolor{red}{(C)}
\end{minipage}}}
\caption{Hypotheses}
\label{tab:hypotheses}
\end{subtable}

\caption{Tabular premise and hypotheses example from \parentDatasetName~ \cite{gupta-etal-2020-infotabs}} 
\label{fig:example} 
\end{figure}

% \end{document}


==> common.tex <==
\usepackage{xspace}
\newcommand{\datasetName}{{\sc MsIn-InfoTabS}\xspace}
\newcommand{\parentDatasetName}{{\sc InfoTabS}\xspace}
\newcommand{\contra}{{\textcolor{red}{\textbf{C}}}\xspace}
\newcommand{\neutral}{{\textcolor{gray}{\textbf{N}}}\xspace}
\newcommand{\entailment}{{\textcolor{cadmiumgreen}{\textbf{E}}}\xspace}
\newcommand{\paperTitle}{\datasetName: Exploring Multi-Set Inoculation on Semi-Structured Tables }

\newcommand{\bert}{{\sc BERT}\xspace}
\newcommand{\roberta}{{\sc RoBERTa}\xspace}
\newcommand{\robertaL}{{\sc RoBERTa-Large}\xspace}
\newcommand{\model}{{\sc RoBERTa$_{\text{\sc InfoTabs}}$}\xspace}
\usepackage{paralist}
\usepackage[review]{lrec-coling2024}

==> conf-matrices.tex <==
\subsection{{\sc OP$_{\text{ZS}}$}}
\newcommand{\method}{{\sc OP$_{\text{ZS}}$} }


Key used as show in Table~\ref{table:perturbation-desc}.
\newcommand{\modelmeth}{Flan-T5-Small }

\subsubsection{Results on \modelmeth}
\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
  \begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opzs/conf-matrix-flan-t5-small-df\var test-unperturbed.png}
    \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
    \label{fig:\var flan t5 small opzs unperturbed}
  \end{figure}
}

\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
  \begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opzs/conf-matrix-flan-t5-small-df\var test-perturbed.png}
    \caption{Results on \var { }perturbed set R$_\short$ for \method method on \modelmeth.}
    \label{fig:\var flan t5 small opzs perturbed}
  \end{figure}
}

\renewcommand{\modelmeth}{Flan-T5-XXL }

\subsubsection{Results on \modelmeth}
\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opzs/conf-matrix-flan-t5-xxl-df\var test-unperturbed.png}
    \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
    \label{fig:\var flan t5 xxl opzs unperturbed}
  \end{figure}
}

\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
\begin{figure}[ht]
  \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opzs/conf-matrix-flan-t5-xxl-df\var test-perturbed.png}
    \caption{Results on \var { }perturbed set R$_\short$ for \method method on \modelmeth.}
    \label{fig:\var flan t5 xxl opzs perturbed}
  \end{figure}
}

\renewcommand{\modelmeth}{GPT-3.5 }
\subsubsection{Results on \modelmeth}
\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opzs/conf-matrix-gpt-3.5-turbo-df\var test-unperturbed.png}
    \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
    \label{fig:\var gpt3.5 opzs unperturbed}
  \end{figure}
}

\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
\begin{figure}[!htb]
\centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opzs/conf-matrix-gpt-3.5-turbo-df\var test-perturbed.png}
    \caption{Results on \var { }perturbed set R$_\short$ for \method method on \modelmeth.}
    \label{fig:\var gpt3.5 opzs perturbed}
  \end{figure}
}



\subsection{{\sc OP$_{\text{COT}}$}}
\renewcommand{\method}{{\sc OP$_{\text{COT}}$} }


Key used as show in Table~\ref{table:perturbation-desc}.
\renewcommand{\modelmeth}{GPT-3.5 }
\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
\begin{figure}
\centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opcot/conf-matrix-gpt-3.5-turbo-df\var test-unperturbed.png}
    \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
    \label{fig:\var gpt3.5 opcot unperturbed}
  \end{figure}
}

\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/opcot/conf-matrix-gpt-3.5-turbo-df\var test-perturbed.png}
    \caption{Results on \var { }perturbed set R$_\short$ for \method method on \modelmeth.}
    \label{fig:\var gpt3.5 opcot perturbed}
  \end{figure}
}




\subsection{{\sc MESP$_{\text{MPI}}$}}
\renewcommand{\method}{{\sc MESP$_{\text{MPI}}$} }
\renewcommand{\modelmeth}{GPT-3.5 }
\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
  \begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/mespmpi/gpt-\var -unp.png}
    \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
    \label{fig:\var gpt3.5 mespmpi unperturbed}
  \end{figure}
}
\foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
  \begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/mespmpi/gpt-\var -p.png}
    \caption{Results on \var { }perturbed set R$_\short$ for \method method on \modelmeth.}
    \label{fig:\var gpt3.5 mespmpi perturbed}
  \end{figure}
}

% \subsection{{\sc MESP$_{\text{MPE}}$}}
% \renewcommand{\method}{{\sc MESP$_{\text{MPE}}$} }
% \renewcommand{\modelmeth}{GPT-3.5 }


% \foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
%   \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/mespmpe/gpt-\var -unp.png}
%     \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
%     \label{fig:\var gpt3.5 mespmpe unperturbed}
%   \end{figure}
% }


% \foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
%   \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/mespmpe/gpt-\var -p.png}
%     \caption{Results on \var { }perturbed set R$_\short$ for \method method on \modelmeth.}
%     \label{fig:\var gpt3.5 mespmpe perturbed}
%   \end{figure}
% }



% % \subsection{Roberta-Large}
% % \subsubsection{Baseline}
% % \newcommand{\method}{Baseline }
% % \newcommand{\modelmeth}{roberta }

% % \foreach \var/\short in {char/C,neg/N,loc/L,stan/S,num/M}{
% %   \begin{figure}[H]
% %     \centering
% %     \includegraphics[width=0.9\linewidth]{Multi-Set-Innoculation/conf-matrices/roberta-large/baseline/conf-matrix-flan-t5-xxl-df\var test-unperturbed.png}
% %     \caption{Results on \var { }unperturbed set R'$_\short$ for \method method on \modelmeth.}
% %     \label{fig:\var flan t5 xxl opzs unperturbed}
% %   \end{figure}
% % }




==> msin-strategies.tex <==
\renewcommand{\arraystretch}{1.5} % Adjust the value to increase or decrease row spacing
\begin{table*}
\footnotesize
\renewcommand{\arraystretch}{1}
    \centering

    \setlength{\tabcolsep}{1.75pt} % Adjust the spacing between columns

    \scalebox{0.85}{\begin{tabular}{p{2.75cm} p{1.5cm} p{14cm}}
    \toprule
    \textbf{Strategy} & \textbf{Abbr.} & \textbf{Strategy Description} \\
    \midrule
     Sequential & {\sc Seq} & Fine-tuning on a $k$ samples from different types of perturbations sequentially {\sc P}$_{1},$ {\sc P}$_{2}, \ldots ${\sc P}$_{N}$, in order, i.e, model is finetuned on samples from {\sc P}$_{1}$ first then {\sc P}$_{2}$ and so on.\\
     Mixed-Training & {\sc Mix}& Fine-tuning using a mixture of $mk$ instances from all challenge sets, where $k$ samples are chosen from each \sc P$_{i}$.  \\
     Dynamic Mixed \newline -Training & {\sc DynMix}&  Similar to {\sc MIX}, except unequal number of samples $\{k_1,k_2,\ldots,k_n\}$ from $\{${\sc P}$_1,${\sc P}$_2 \ldots ${\sc P}$_m\}$ are used for fine-tuning. The number of samples $k_i$'s are inversely proportional to the baseline performance on set {a \sc P}$_i$.
    % Fine-Tuning using a mixture of $k_1+k_2+k_3\ldots+k_n \in P_{mix}$ samples obtained by taking $k_1$ examples from $P_1$,$k_2$ from $P_2$ and so on.  $P_{mix}=P_{1} \cup P_{2} \cup P_{3}, \ldots \cup P_{N}$ On model $M$ trained for $D$ for a given task $T$, if a perturbation $\pi_{i}$ is tougher than $\pi_{j}$, we typically select more examples from $P_{i}$ than $P_{j}$.  
    \\
    %\midrule
    % \textbf{Prompt Engineering} & 
     Original Prompt \newline with COT& {\sc OP$_{\text{COT}}$} & The constructed prompt consists of a description of task {\sc T} with demonstrations of the unperturbed set {\sc O}  in the prompt along with reasoning. \\
    Mixed-Prompting-Instructional  & {\sc MESP$_{\text{MPI}}$} & The constructed prompt consists of a description of task {\sc T} with a verbose description of each type of perturbations with at least 1 demonstration from each perturbation type $\pi_i$ and from the original set {\sc O}. \\
    Mixed-Prompting-Exemplar  & {\sc MESP$_{\text{MPE}}$} & The constructed prompt consists of a description of task {\sc T} with a brief description of each type of perturbation with multiple demonstrations from each perturbation type $\pi_i$ and from the original set {\sc O}.
    \\
    % For a general prompt-based model (\textit{LLMs}) $M$ We create a prompt format describing the nature and scope of task $T$ and a verbose description of the types of perturbations ( $P_{1}, P_{2}, P_{3}, \ldots$.) that can occur along with a few examples from the unperturbed set $D$ and a few from each of the perturbed sets($P_{1}, P_{2}, P_{3}, \ldots$.) along with reasoning, here we attempt to explain the perturbation and attempt to make $M$ understand the scope of perturbations through instructions. 
    %& Mixed-Prompting-Exemplar & $\mathit{MIXEXM}$ & For a general prompt-based model (\textit{LLMs}) $M$ We create a prompt format describing the nature and scope of task $T$ and a brief (short) description of the types of perturbations ( $P_{1}, P_{2}, P_{3}, \ldots$.) that can occur along with many examples from the unperturbed set $D$ and many from each of the perturbed sets($P_{1}, P_{2}, P_{3}, \ldots$.) along with reasoning. Here we try to focus on making $M$ understand the scope of perturbations through examples. \\
    \bottomrule
    \end{tabular}}
    \vspace{-0.5em}
    \caption{\textbf{Strategies for Multi-Set Inoculation for PLMs} }
    \label{table:msin-strats}
    \vspace{-1.0em}
\end{table*}


%\renewcommand{\arraystretch}{1.5} % Adjust the value to increase or decrease row spacing
%\begin{table*}
    %\centering

    %\setlength{\tabcolsep}{4pt} % Adjust the spacing between columns

   % \scalebox{0.85}{\begin{tabular}{p{1.5cm} p{2cm} p{1.5cm} p{13cm}}
   % \toprule
   % \textbf{Class} & \textbf{Strategy} & \textbf{Abbr.} & \textbf{Strategy Description} \\
 %   \midrule
 %   \textbf{Fine-tuning} & Sequential & ${\sc Seqt} & Fine-tuning on a $k$ samples from different types of perturbations sequentially $P_{1}, P_{2}, \ldots P_{N}$, in order, i.e, model is fined on samples from $P_{1}$ first then $P_{2}$ and so on.\\
  %  & Mixed & {\sc Mix}& Fine-tuning using a random mixture of $Nk \in P_{mix}$ samples obtained via the union of k samples from each perturbation set.  $P_{mix}=P_{1} \cup P_{2} \cup P_{3}, \ldots \cup P_{N}$. \\
   % & Mixed and Data-size variation & $\mathit{VARYMIX}$ &  Similar to $\mathit{MIXT}$, except unequal number of samples $\{k_1,k_2,\ldots,k_n\}$ from $\{P_1$,$P_2$$\ldotsP_N\}$ are used for fine-tuning. The number of samples $k_i$'s are propotional to reduction in performance with on set $P_i$.
    %Fine-Tuning using a mixture of $k_1+k_2+k_3\ldots+k_n \in P_{mix}$ samples obtained by taking $k_1$ examples from $P_1$,$k_2$ from $P_2$ and so on.  $P_{mix}=P_{1} \cup P_{2} \cup P_{3}, \ldots \cup P_{N}$ On model $M$ trained for $D$ for a given task $T$, if a perturbation $\pi_{i}$ is tougher than $\pi_{j}$, we typically select more examples from $P_{i}$ than $P_{j}$.  
    \\
    %\midrule
    %\textbf{Prompt Engineering} & Unperturbed-COT-Prompting & $\mathit{UNPCOT}$ & For a general prompt-based model (\textit{LLMs}) $M$ We create a prompt format describing the nature and scope of task $T$ and provide some examples (demonstrations) of the unperturbed set $D$  in the prompt along with reasoning. \\
    %& Mixed-Prompting-Instructional & $\mathit{MIXINS}$ & For a general prompt-based model (\textit{LLMs}) $M$ We create a prompt format describing the nature and scope of task $T$ and a verbose description of the types of perturbations ( $P_{1}, P_{2}, P_{3}, \ldots$.) that can occur along with a few examples from the unperturbed set $D$ and a few from each of the perturbed sets($P_{1}, P_{2}, P_{3}, \ldots$.) along with reasoning, here we attempt to explain the perturbation and attempt to make $M$ understand the scope of perturbations through instructions. \\
    %& Mixed-Prompting-Exemplar & $\mathit{MIXEXM}$ & For a general prompt-based model (\textit{LLMs}) $M$ We create a prompt format describing the nature and scope of task $T$ and a brief (short) description of the types of perturbations ( $P_{1}, P_{2}, P_{3}, \ldots$.) that can occur along with many examples from the unperturbed set $D$ and many from each of the perturbed sets($P_{1}, P_{2}, P_{3}, \ldots$.) along with reasoning. Here we try to focus on making $M$ understand the scope of perturbations through examples. \\
%    \bottomrule
%    \end{tabular}}
%    \caption{\textbf{Strategies for Multi-Set Inoculation for PLMs} }
%    \label{table:msin-strats}
%\end{table*}

==> perturbation-descriptions.tex <==

\begin{table}[!htb]
\footnotesize
\renewcommand{\arraystretch}{1}
\centering
\begin{tabular}{lll}
\toprule
\textbf{Class} & \textbf{Key} & \textbf{Type} \\ 
\midrule
char & C & Character-level perturbation \\
neg & N & Negation-type perturbation \\
num & M & Numeric perturbation \\
loc & L & Location perturbation \\
stan & S  & Paraphrasing as a perturbation \\
\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{\textbf{Perturbation Types: } We use 5 distinct perturbations as challenge sets for Tabular-NLI.}
\label{table:perturbation-desc}
\vspace{-1.5em}
\end{table}


==> prompt-engineering-results.tex <==
\vspace{-1.0em}
\subsection{Results: Large Language Models (LLMs)}
\vspace{-0.5em}
% We present results on Zero-Shot({\sc OP$_{\text{ZS}}$}), Few-Shot({\sc OP$_{\text{COT}}$}), Single Exemplars Multiple Prompts ({\sc SEMP}), Multiple Exemplars Single Prompts({\sc MESP}) are shown in table ~\ref{table-llm-ins}, ~\ref{table-unpcot}, ~\ref{table-single-aware-a} and ~\ref{table-mix-llms-llama}.

%\textbf{Original Prompt.}  Table~\ref{table-llm-ins} and \ref{table-unpcot} shows the results for Original Zero-Shot Prompts ({\sc OP$_{\text{ZS}}$}) and Few-shot with CoT({\sc OP$_{\text{CoT}}$}), respectively.\footnote{Results on other open source models in Appendix \ref{sec:appendix_additional_results}.}
\textbf{Original Prompt.}  Table~\ref{llm-op-zs-cot} shows the results for {\sc OP$_{\text{ZS}}$} and {\sc OP$_{\text{CoT}}$}, respectively. Results on other open source models in Appendix \ref{sec:appendix_additional_results}.
%\footnote{Results on other open source models in Appendix \ref{sec:appendix_additional_results}.}
%\vspace{-1em}
\input{tables/table-op-cot-zs}
% \input{tables/table-llm-ins}
%\input{tables/table-unpcot}

\textit{Analysis.} \begin{inparaenum}[(a.)] On the Original Zero-Shot Prompts we observe that, 
    \item Comparing the results of challenge datasets {\sc Q$_j$} and their unperturbed version sets {\sc Q'$_j$} reveals that LLMs similar to PLMs are also sensitive to input data perturbations. 
    \item However, the Flan-T5 series, specifically XL and XXL, performs significantly better than other LLMs as it's fine-tuned specifically for the NLI task \citep{chung2022scaling}. Even the drop in performance due to data perturbation is relatively less.
    \item The poor performance of relatively smaller LLMs, such as LLaMA-2-13b, demonstrates the ineffectiveness of such models in responding to an instruction prompt. %\footnote{LLaMA-2-13b often labeled examples as \textcolor{gray}{Neutral (N),} even with correct reasoning.}.
    \item One reason for performance on original numerical set ({\sc Q'$_M$)}, is due to model inability to handle mathematical reasoning \citep{wallace2019nlp,min2021recent,hendrycks2021measuring,imani-etal-2023-mathprompter}. 
    Additionally, we find that all models enhanced with CoT (Table \ref{llm-op-zs-cot}) outperform those using Zero Shot original prompts. This suggests that simply adding exemplars can enhance a model's resilience to perturbations. 
\end{inparaenum}

 % \noindent 
 \textbf{Single Exemplars Multiple Prompts ({\sc SEMP})}: Table~\ref{table-single-aware-a} presents results for GPT-3.5, with diagonal elements as an analogue to single set inoculation. LLaMA-2 results are in Table~\ref{table-llama-2-single-aware-b}.
 
\input{tables/table-single-aware}
\vspace{-1em}
% \input{tables/table-llama-2-single-aware}
\textit{Analysis.} From Tables~\ref{table-single-aware-a} and~\ref{table-llama-2-single-aware-b}, it's evident that incorporating an input perturbation explanation within the prompt enhances the model's accuracy. The results in Table ~\ref{table-single-aware-a} suggest that even a singular perturbation explanation prompts the model to anticipate other perturbations, essentially priming it for a noisy environment. This adaptability is especially pronounced for character perturbations, where improvements span across all challenge sets. Comparisons with instructional prompts and few-shot results show that demonstrations with perturbation explanations improve performance.

%We note a correlation between semantic (N, S) perturbations, which modify sentence meaning, and syntactic (C, M, L) perturbations, which alter specific words in a sentence. Demonstrations from {\sc P$_C$} prompt the model to refine the hypothesis before drawing an inference, leading to notable improvements in {\sc R$_C$}, {\sc R$_M$}, and {\sc R$_L$}. Similarly, when provided with details about $\pi_S$, we see marked performance gains on {\sc R$_N$}.
% \noindent 
\input{tables/table-mix-llms-llama}
\textbf{Multiple Exemplars Single Prompts ({\sc MESP})}: The results for \textbf{MPI} and \textbf{MPE} are in Table~\ref{table-mix-llms-gpt-llama}.

% \input{tables/table-mix-llms-llama}

\textit{Analysis.} Both models show marked improvement with mixed prompting, indicating that LLMs, when guided with perturbation descriptions and examples, yield more stable outputs. The superior performance of MPE over MPI suggests that including more examples in prompts is more beneficial than detailed perturbation descriptions.

In conclusion, LLMs too face challenges with input perturbations. Simply explaining one perturbation primes the LLM to consider others.  Our findings show that a mixed prompting approach with several perturbation instances and brief explanations improves robustness.

% \vk{}

% \noindent 
% \textbf{Fine-tuning GPT-3.5:}
% \label{fine_tune_sec}
% We report fine-tuning of GPT-3.5 results in Table~\ref{tab:fine_tuning}. This included taking 50 examples from each of the perturbed sets ${\text{{\sc P}}_j}$ and 50 from the unperturbed set $ \bigcup {\text{{\sc P'}}_j}$ and fine-tuning the model.
% \input{tables/table-fine-tuning}
% Mixed fine-tuning outperforms prompts with perturbed exemplars by approximately 7 points. Thus, fine-tuning on perturbed cases improves LLM resilience to input perturbation too. We exclusively compare our results with \textbf{\textsc{MESP}}$_{\text{\textbf{MPE}}}$, which is the preferred approach, as elaborated in \S \ref{sec:results_roberta}. %We report on GPT-3.5 fine-tuning since it beats other models and fits our computing budget.

\textbf{Fine-tuning on LLMs.}
\label{fine_tune_sec}
While our paper primarily focuses on in-context learning for LLMs, we also examine the effects of fine-tuning LLMs on perturbation sets, results shown in Table ~\ref{tab:fine_tuning_LLM}. We can see that for Mixtral and GPT-3.5 the fine tuning with the perturbation set using the mix training approach increases the models' performance. Whereas for the Flan-T5-L model the fine tuning does not improve the model's performance. 
\input{tables/fine_tuning_LLLM}

==> tables/TableExample.tex <==
% % \begin{table}[!ht]
% % \small
% % \renewcommand{\arraystretch}{1} % Adjust the value as needed
% % \centering
% % \begin{tabularx}{\linewidth}{l X}
% %   \toprule
% %   \multicolumn{2}{c}{\textbf{Case Closed}} \\
% %   \midrule
% %   \textbf{Written by} & Takahiro Arai \\
% %   \textbf{Published by} & Shogakukan \\
% %   \textbf{English publisher} & SG Shogakukan Asia \\
% %   \textbf{Demographic} & Shonen \\
% %   \textbf{Magazine} & Weekly Shonen Sunday \\
% %   \textbf{Original run} & May 9, 2018 - present \\
% %   \textbf{Volumes} & 2 (List of volumes) \\
% %  \bottomrule
% %  \multicolumn{2}{l}{{\textbf{H1}}: 'Case Closed' was written by Takahiro Arai and}\\
% %  \multicolumn{2}{l}{ published by Shogakukan. \textcolor{cadmiumgreen}{(E)}}\\
% %  \multicolumn{2}{l}{{\textbf{H1'}}: 'Case Closed' was writtKen b Takhahiro Arai }\\
% %  \multicolumn{2}{l}{and publihsed by Shogakukn.\textcolor{cadmiumgreen}{(E)}}\\
% %  \hline
% %  \multicolumn{2}{l}{{\textbf{H2}}: 'Case Closed' was a long-running Japanese }\\
% %   \multicolumn{2}{l}{comic serial.\textcolor{cadmiumgreen}{(E)}}\\
% %   \multicolumn{2}{l}{{\textbf{H2'}}: 'Case Closed' was not a long-running Japanese }\\
% %   \multicolumn{2}{l}{comic serial.\textcolor{red}{(C)}}\\
% %   \hline
% %   \multicolumn{2}{l}{{\textbf{H3}}: 'Case Closed' was made into an anime called} \\
% %   \multicolumn{2}{l}{Detective Conan.\textcolor{gray}{(N)}}\\
% %   \multicolumn{2}{l}{{\textbf{H3'}}: Detective Conan was an anime adaptation} \\
% %   \multicolumn{2}{l}{of 'Case Closed'.\textcolor{gray}{(N)}} \\
% %   \hline
% %     \multicolumn{2}{l}{{\textbf{H4}}: 'Case Closed' has been running for more than} \\
% %   \multicolumn{2}{l}{5 years\textcolor{cadmiumgreen}{(E)}}\\
% %   \multicolumn{2}{l}{{\textbf{H4'}}: 'Case Closed' has been running for more than} \\
% %   \multicolumn{2}{l}{10 years\textcolor{red}{(C)}}\\
% %   \hline
% %    \multicolumn{2}{l}{{\textbf{H5}}: 'Case Closed' was published in English by SG } \\
% %   \multicolumn{2}{l}{Shogakukan Asia\textcolor{cadmiumgreen}{(E)}}\\
% %   \multicolumn{2}{l}{{\textbf{H5'}}: 'Case Closed' was published in English by SG} \\
% %     \multicolumn{2}{l}{Shogakukan Australia\textcolor{red}{(C)}}\\
% % \end{tabularx}
% % \caption{\textbf{An example of tabular premise and hypotheses from \parentDatasetName~ \cite{gupta-etal-2020-infotabs}.}
% % Original hypotheses (H1,H2,H3,H4,H5) and perturbed hypothesis \textbf{(H1',H2',H3',H4',H5')} representing character,negation,paraphrasing,numeric and location perturbations respectively. 
% % \\ Labelled as \textcolor{cadmiumgreen}{E}ntailment,\textcolor{red}{C}ontradiction or \textcolor{gray}{N}eutral.
% % \\ 
% % The \textbf{bold} entries, which correspond to the first column, are the keys, while the corresponding entries in the second column of the same row are their respective values.}
% % \label{tab:example}
% % \end{table}


% \begin{table}
% %\begin{center}
% \centering
% \renewcommand{\arraystretch}{1}
% \footnotesize{
% \begin{tabular}{l l}\\
% \hline
% \multicolumn{2}{c}{\textbf{Case Closed}} \\
% \hline
%   \textbf{Written} & Takahiro Arai \\ 
%   \textbf{Publish} & Shogakukan \\
%   \textbf{Eng. Publish} & SG Shogakukan Asia \\
%   \textbf{Demographic} & Shonen \\
%   \textbf{Magazine} & Weekly Shonen Sunday \\
%   \textbf{Orig. Run} & May 9, 2018 - present \\
%   \textbf{Volumes} & 2 (List of volumes) \\
% \hline
% \end{tabular}}
% % \end{subtable}
% %\end{center}
% \begin{tabular}{cc}
% %\centering
% \begin{center}
% \footnotesize 
% {
% \fbox{\begin{minipage}{43em}
%     %\textbf{H$_1$:} Takahiro Arai wrote `Case Closed' comic series. \textcolor{cadmiumgreen}{(E)} \\
%     %\textbf{H$_1^'$:} Takahiro Arai wotte `Case Closed' comci series. \textcolor{cadmiumgreen}{(E)} \\
%     %\textbf{H$_2$:} `Case Closed' is a long-term comic series. \textcolor{cadmiumgreen}{(E)} \\
%     %\textbf{H$_2^'$:}  `Case Closed' isn't a long-term comic series.  \textcolor{red}{(C)} \\
%     %\textbf{H$_3$:} `Case Closed' became the anime Detective Conan \textcolor{gray}{(N)} \\
%     %\textbf{H$_3^'$:} Detective Conan is `Case Closed' anime version. \textcolor{gray}{(N)} \\
%     %\textbf{H$_4$:}  `Case Closed' has run over 5 years.\textcolor{cadmiumgreen}{(E)} \\
%     %\textbf{H$_4^'$:} `Case Closed' has run over 10 years.\textcolor{red}{(C)} \\ 
%     %\textbf{H$_5$:} Shogakukan Asia published `Case Closed' (Eng). \textcolor{cadmiumgreen}{(E)}\\ 
%     %\textbf{H$_5^'$:}  Shogakukan UK published `Case Closed' (Eng). \textcolor{red}{(C)}
% \end{minipage}}} 
% \end{center}
% \end{tabular}
% \vspace{-0.5em}
% %\caption{\small{Tabular premise and hypotheses example from \parentDatasetName ~\cite{gupta-etal-2020-infotabs}. Original (H$_1$-H$_5$) and perturbed hypotheses (H$_1^'$-H$_5^'$) represent character, negation, paraphrasing, numeric, and location perturbations. Labeled as \textcolor{cadmiumgreen}{E}, \textcolor{red}{C}, or \textcolor{gray}{N}. \textbf{Bold} entries are keys; adjacent entries are their values.}}
% % \caption{\small \textbf{An example of tabular premise and hypotheses from \parentDatasetName~ \cite{gupta-etal-2020-infotabs}.}
% % Original hypotheses (H1,H2,H3,H4,H5) and perturbed hypothesis \textbf{(H1',H2',H3',H4',H5')} representing character,negation,paraphrasing,numeric and location perturbations respectively.  Labelled as \textcolor{cadmiumgreen}{E}ntailment,\textcolor{red}{C}ontradiction or \textcolor{gray}{N}eutral. The \textbf{bold} entries, which correspond to the first column, are the keys, while the corresponding entries in the second column of the same row are their respective values.} 
% \vspace{-1.75em}
% \label{tab:example}
% \end{table}


\begin{figure} 
\centering 
\begin{subtable}[b]{0.45\textwidth} 
\centering
\renewcommand{\arraystretch}{1}
\footnotesize{
\begin{tabular}{l l}\\
\hline
\multicolumn{2}{c}{\textbf{Case Closed}} \\
\hline
\textbf{Written} & Takahiro Arai \\
\textbf{Publish} & Shogakukan \\
\textbf{Eng. Publish} & SG Shogakukan Asia \\
\textbf{Demographic} & Shonen \\
\textbf{Magazine} & Weekly Shonen Sunday \\
\textbf{Orig. Run} & May 9, 2018 - present \\
\textbf{Volumes} & 2 (List of volumes) \\
\hline
\end{tabular}}
%\caption{Case Closed Details} 
%\label{tab:case_details}
\hspace{-2em}
\end{subtable}
\hfill 
\begin{subtable}[b]{0.45\textwidth}  
\centering
\footnotesize
{
\fbox{\begin{minipage}{25em}
\textbf{H$_1$:} Takahiro Arai wrote `Case Closed' comic series. \textcolor{cadmiumgreen}{(E)} \\
\textbf{H$_1^'$:} Takahiro Arai wotte `Case Closed' comci series. \textcolor{cadmiumgreen}{(E)}
\\
\textbf{H$_2$:} `Case Closed' is a long-term comic series.\textcolor{cadmiumgreen}{(E)}
\\
\textbf{H$_2^'$:}`Case Closed' isn't a long-term comic series.\textcolor{red}{(C)} \\
\textbf{H$_3$:}`Case Closed' became the anime Detective Conan \textcolor{gray}{(N)} \\
\textbf{H$_3^'$:}Detective Conan is `Case Closed' anime version. \textcolor{gray}{(N)} \\
\textbf{H$_4$:}`Case Closed' has run over 5 years.\textcolor{cadmiumgreen}{(E)} \\
\textbf{H$_4^'$:}`Case Closed' has run over 10 years.\textcolor{red}{(C)} \\
\textbf{H$_5$:} Shogakukan Asia published `Case Closed' (Eng). \textcolor{cadmiumgreen}{(E)}\\ 
\textbf{H$_5^'$:}Shogakukan UK published `Case Closed' (Eng). \textcolor{red}{(C)}
\end{minipage}}}
%\caption{Hypotheses}
\label{tab:hypotheses}
\end{subtable}

\caption{Tabular premise and hypotheses example from \parentDatasetName~ \cite{gupta-etal-2020-infotabs}} 
\label{fig:example} 
\end{figure}

==> tables/fine_tuning_LLLM.tex <==
\begin{table}[!ht]
 \vspace{-0.25em}
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{5.8pt} % Adjust the spacing between columns
\scalebox{0.80}{
\begin{tabular}{l|c|cccccc}
% \hline
    % & \multicolumn{5}{c}{\textbf{\textsc{Metrics}}} & \textbf{\textsc{Avg.}} \\
% \hline
&\textbf{Model} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & \textbf{avg.} \\
\cline{2-8}
\multirow{3}{*}{\begin{sideways}\textbf{BASE}\end{sideways}} 
& Flan-t5-L & 63.00 & 70.00 & 63.00 & 65.00 & 69.30 & 66.06 \\
& Mistral & 44.01 & 39.66 & 23.67 & 41.34 & 39.67 & 37.67 \\
& GPT-3.5 & 51.00 & 53.00 & 62.66 & 61.00 & 60.30 & 57.59 \\
\hline
\multirow{3}{*}{\begin{sideways}\textbf{FT}\end{sideways}} 
& Flan-t5-L & 51.71 & 27.77 & 45.31 & 42.71 & 58.70 & 45.24 \\
& Mistral & 43.67 & 39.00 & \textbf{61.67} & 45.67 & 44.34 & 46.87 \\
& GPT-3.5 & \textbf{71.67} & \textbf{78.33} & \textbf{66.67} & \textbf{67.33} & \textbf{71.00} & \textbf{71.00} \\
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{Fine tuning results for Flan-T5-L-0.8b, Mistral-7b-instruct-v0.2 and GPT-3.5-turbo on perturbed sets and average of performance.
\textit{FT refers to Fine-Tuning results and BASE refers to {\sc OP$_{\text{ZS}}$} results.}}
\vspace{-1.0em}
\label{tab:fine_tuning_LLM}
\end{table}


==> tables/in-out-1-table.tex <==
\begin{table}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt} % Adjust the spacing between columns
    \begin{tabular}{l|ccc|cc|ccc|c}
        & \multicolumn{3}{c|}{\textbf{In-distribution}} & \multicolumn{2}{c|}{\textbf{Out-distribution}} & \multicolumn{3}{c|}{\textbf{Original Test sets}} & \\
        \cline{1-10}
        \textbf{K} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{char} & \textbf{stan} & \textbf{alpha1} & \textbf{alpha2} & \textbf{alpha3} & \textbf{$\mu$} \\
        \hline
        \textbf{baseline} & 46.90 & 67.20 & 70.20 & 57.30 & 67.10 & 72.72 & 64.83 & 62.33 & - \\
        \textbf{100} & 60.4 & 83.2 & 81.4 & 49.6 & 59.6 & 63.6 & 62.8 & 56.1 & 51.0 \\
        \textbf{200} & 61.9 & 85.6 & 83.0 & 49.2 & 58.0 & 61.3 & 61.9 & 53.0 & 57.9 \\
        \textbf{300} & 62.1 & 85.8 & 83.2 & 48.8 & 55.7 & 59.4 & 62.3 & 51.9 & 53.9 \\
        \textbf{400} & 66.3 & 85.1 & 83.5 & 47.5 & 54.3 & 58.4 & 61.5 & 51.1 & 56.1 \\
        \textbf{500} & 68.0 & 86.0 & 84.1 & 47.8 & 53.9 & 58.0 & 61.2 & 50.1 & 62.3 \\
        \hline
    \end{tabular}
    \caption{In-distribution represents perturbation types used for training, In-distribution are the other perturbation types. K is the number of samples used for each perturbation during training. $\mu$ is the average improvement over the baseline of all perturbation sets.}
    \label{tab:in-out-1}
\end{table}

==> tables/in-out-2-table.tex <==
\begin{table}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt} % Adjust the spacing between columns
    \begin{tabular}{c|cc|ccc|ccc|c}
        & \multicolumn{2}{c|}{\textbf{In-distribution}} & \multicolumn{3}{c|}{\textbf{Out-distribution}} & \multicolumn{3}{c|}{\textbf{Original Test sets}} & \\
        \cline{1-10}
        \textbf{K} & \textbf{char} & \textbf{num} & \textbf{neg} & \textbf{loc} & \textbf{stan} & \textbf{alpha1} & \textbf{alpha2} & \textbf{alpha3} & \textbf{avg.} \\
        \hline
        \textbf{baseline} & 57.30 & 67.20 & 46.90 & 70.20 & 67.10 & 72.72 & 64.83 & 62.33 & - \\
        \textbf{100} & 56.3 & 80.1 & 50.3 & 74.6 & 65.4 & 71.0 & 63.2 & 60.1 & 36.1 \\
        \textbf{200} & 57.2 & 82.8 & 47.9 & 76.3 & 65.3 & 70.9 & 63.5 & 59.2 & 41.5 \\
        \textbf{300} & 57.0 & 83.1 & 47.0 & 77.1 & 65.2 & 71.1 & 63.1 & 58.1 & 41.3 \\
        \textbf{400} & 58.0 & 84.1 & 48.5 & 78.0 & 64.4 & 70.8 & 63.8 & 58.4 & 48.6 \\
        \textbf{500} & 57.0 & 84.1 & 46.7 & 77.7 & 64.4 & 70.9 & 63.2 & 58.0 & 42.5 \\
        \hline
    \end{tabular}
    \caption{In-distribution represents perturbation types used for training, In-distribution are the other perturbation types. K is the number of samples used for each perturbation during training. $\mu$ is the average improvement over the baseline of all perturbation sets.}
    \label{tab:in-out-2}
\end{table}

==> tables/table-cross-testing-roberta-large.tex <==


\begin{table}[!ht]
\renewcommand{\arraystretch}{1.1}
    \centering
    \small
    \setlength{\tabcolsep}{2.75pt} % Adjust the spacing between columns
    \scalebox{0.85}{
        \begin{tabular}{@{}l|ccc|ccccc}
            \hline
            \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Original Test Sets}} & \multicolumn{5}{c}{\textbf{Challenge Test Sets}} \\
            \hline
            \diagbox[innerwidth=1.4cm, height=0.8cm]{\textbf{Train}}{\textbf{Test}} & $\boldsymbol{\alpha_1}$ & $\boldsymbol{\alpha_2}$ & $\boldsymbol{\alpha_3}$ & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} \\
            \hline
            baseline &72.72 & \bf 64.83 & 62.33 & 57.30 & 46.90 & 67.20 & 70.20 & 67.10 \\
            \hline
            char & \bf 75.28 & 63.83 & \bf 63.33 & \textbf{59.20} & 43.70 & 64.30 & 66.00 & \bf 68.30 \\
            neg & 66.94 & 64.56 & 58.06 & 52.80 & \textbf{71.90} & 69.60 & 69.70 & 62.40 \\
            num & 62.06 & 60.83 & 52.50 & 47.30 & 49.60 & \textbf{85.40} & 83.00 & 57.60 \\
            loc & 55.78 & 58.67 & 49.67 & 47.40 & 53.90 & 84.60 & \textbf{86.10} & 53.50 \\
            stan & 73.56 & 62.61 & 60.44 & 58.30 & 40.80 & 70.30 & 67.80 & 66.80 \\
            \hline
        \end{tabular}
    }
\vspace{-0.5em}
\caption{\textbf{Multi-model Uniset Inoculation:} \model when fine-tuned on one of the challenge sets({\sc P}$_i$), but tested on all challenge sets ({\sc Q}$_i$) with number of sample used equal 500. }
\vspace{-1.0em}
    \label{table-cross-testing-roberta-large}
\end{table}

==> tables/table-fine-tuning.tex <==
\begin{table}[!ht]
    \vspace{-0.5em}
    \centering
    \small
    \setlength{\tabcolsep}{8pt} % Adjust the spacing between columns
    \scalebox{0.85}{
    \begin{tabular}{l|cccccc}
        \hline
        \textbf{Model} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & \textbf{Q'} \\
        \hline
        \textbf{Base} &51.00 & 53.00 &  62.66 & 61.00 & 60.30 & 69.45\\
        \hline
        \textbf{\textsc{MESP}}$_{\text{\textbf{MPE}}}$ & 70.00 & 63.60 & 58.30 & 60.00 & 66.80 & 72.52 \\
        % \hline
        \textbf{Fine-Tune} & \bf 71.67 & \bf 78.33 & \bf 66.67 & \bf 67.33 & \bf 71.00 & \bf 76.40 \\
        \hline
    \end{tabular}}
    \vspace{-0.5em}
    \caption{\textbf{GPT-3.5} fine-tuning using {\sc Mix}.}
    \label{tab:fine_tuning}
    \vspace{-1.2em}
\end{table}

==> tables/table-llama-2-single-aware.tex <==
\begin{table}[!ht]
\vspace{-0.25em}
\centering
\small
\setlength{\tabcolsep}{3pt} % Adjust the spacing between columns
\scalebox{0.9}{
\begin{tabular}{p{0.85cm}|c|ccccc}
\hline
%\diagbox[innerwidth=1.5cm, height=0.8cm]{\textbf{set}}{\textbf{$\pi_j$}} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} \\
Type &\textbf{set/\ {$\pi_j$}} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} \\
\hline
\multirow{2}{=}{\textbf{BASE}} 
&{\sc R}$'_j$  & 59.00 & 63.60 & 64.60 & 67.00 & 60.00\\
&{\sc R}$_j$ & 54.00 & 51.60 & 49.60 & 57.00 & 54.30\\ 
\hline
\multirow{2}{=}{\textbf{SEMP}} 
&{\sc R}$'_j$ & 69.00 & 71.00 & 72.00 & 72.30 & 68.60 \\ 
&{\sc R}$_j$ & 53.00 & 58.00 & 62.00 & 62.00 & 68.30 \\ \hline 
\end{tabular}}
\vspace{-0.5em}
\caption{\textbf{SEMP LLaMA-2-70b:}  Self-testing on perturbation $\pi_j$ with prompt for $\pi_j$ and test on {\sc{R$_j$}} and {\sc{R$'_j$}}.}
%\vspace{-1.5em}
\label{table-llama-2-single-aware}
\end{table}


==> tables/table-llm-ins.tex <==
\begin{table}[!ht]
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{6pt} % Adjust the spacing between columns
\scalebox{0.80}{
\begin{tabular}{p{0.25cm}|l|cccccc|cccccccc}
&&  \multicolumn{6}{c|}{\bf Q' } &  \multicolumn{6}{c}{\bf Q } \\

\hline
&\textbf{Model} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & \textbf{avg.} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & \textbf{avg.} \\
\hline
\multirow{3}{=}{\begin{sideways}\textbf{{\sc OP$_{\text{ZS}}$}}\end{sideways}}
&Flan-t5-XXL & \textbf{70.60} & \textbf{77.30} & \textbf{69.00} & \textbf{74.00} & \textbf{79.00} & \textbf{73.98} & \textbf{63.00} & \textbf{70.00} & \textbf{63.00} & \textbf{65.00} & \textbf{69.30} & 66.06 \\
&LLaMA-2-70b & 59.00 & 63.60 & 64.60 & 67.00 & 60.00 & 62.84 & 54.00 & 51.60 & 49.60 & 57.00 & 54.30 & 53.30 \\
&GPT-3.5 & 68.00 & 69.00 & 68.66 & 71.60 & 70.00 & 69.45 & 51.00 & 53.00 & 62.66 & 61.00 & 60.30 & 57.59 \\
\hline
\end{tabular}}
\caption{\textbf{Zero Shot and Few-shot with CoT Results:} Baseline accuracy for LLMs for Original prompts in zero-shot setting.}
\vspace{-1.0em}
\label{table-llm-ins}
\end{table}


==> tables/table-mix-llms-llama.tex <==
\begin{table}[!ht]
\vspace{-0.5em}
\renewcommand{\arraystretch}{1.5}
\centering
\small
\setlength{\tabcolsep}{4pt} % Adjust the spacing between columns
\scalebox{0.85}{ 
\begin{tabular}{l|c|cccccc}
\hline
 & Strategy & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & $R'$ \\
\hline
\multirow{3}{*}{\begin{sideways}\textbf{LLaMA-2}\end{sideways}} 
& \textbf{Base} & 39.67 & 39.33 & 45.67 & 56.67 & 44.67 & 45.20 \\  
& \textbf{\textsc{MESP}$_{\text{MPI}}$} & 58.33 & 51.33 & \textbf{59.67} & 55.00 & \textbf{62.33} & 62.53 \\ 
& \textbf{\textsc{MESP}$_{\text{MPE}}$} & \textbf{60.97} & \textbf{56.67} & 59.33 & \textbf{60.67} & 62.00 & \textbf{65.67} \\ 
\hline
\multirow{3}{*}{\begin{sideways}\textbf{GPT-3.5}\end{sideways}} 
& \textbf{Base} & 51.00 & 53.00 & \textbf{62.66} & \textbf{61.00} & 60.30 & 69.45 \\  
& \textbf{\textsc{MESP}$_{\text{MPI}}$} & 59.60 & \textbf{65.30} & 62.00 & 59.00 & 59.60 & 68.76 \\ 
& \textbf{\textsc{MESP}$_{\text{MPE}}$} & \textbf{70.00} & 63.60 & 58.30 & 60.00 & \textbf{66.80} & \textbf{72.52} \\ 
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{\textbf{MESP Results on LLaMA-2-13b and GPT-3.5}.\textit{LLaMA-2 refers to LLaMA-2-13b.}}
\label{table-mix-llms-gpt-llama} % A descriptive label is always helpful 
\vspace{-0.75em}
\end{table}

==> tables/table-mixed-roberta-large.tex <==
\begin{table}[!ht]
    \centering
     \small
    \setlength{\tabcolsep}{2pt} % Adjust the spacing between columns
    \scalebox{0.85}{
    \begin{tabular}{l|cccccccccc}
        \hline
        \textbf{seed} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} &  \textbf{$\alpha_1$} & \textbf{$\alpha_2$} & \textbf{$\alpha_3$} \\
        \hline
        97 & 0.55 & 0.66 & 0.83 & 0.80 & 0.65 & 0.72 & 0.64 & 0.58 \\
        13 & 0.58 & 0.66 & 0.82 & 0.82 & 0.66 & 0.73 & 0.64 & 0.59 \\
        50 & 0.57 & 0.67 & 0.82 & 0.81 & 0.65 & 0.73 & 0.64 & 0.59 \\
        70 & 0.59 & 0.64 & 0.82 & 0.79 & 0.66 & 0.73 & 0.65 & 0.60 \\
        30 & 0.56 & 0.68 & 0.80 & 0.80 & 0.66 & 0.73 & 0.64 & 0.60 \\
        \hline
    \end{tabular}}
\end{table}


==> tables/table-prompt-example.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{3pt} % Adjust the spacing between columns
\scalebox{0.76}{
\begin{tabular}{@{}p{2.4cm}|p{7.2cm}@{}}
\hline
\multicolumn{2}{c}{\bf Broad Prompt Template}\\
% Broad Template \\
\hline
\textbf{NLI Task Explanation} & In this task, we will ask you to make an inference about the information presented as the premise. We will show you a premise and a hypothesis... \\
\hline
\textbf{Perturbation Awareness} & The concept of numeric and character typos in questions is important for maintaining the integrity and meaning of a sentence... \\
\hline
\textbf{Description of Limitation} & It is very important and critical that you do not use information other than the premise that you may know if you believe that it is not generally known... \\
\hline
\textbf{Answering} & (Restriction for Answering) Answer with an explanation in the following format, restricting the answer to only one of the following: "yes" or "no" or "it is not possible to tell" + Answering Format \\
\hline
\textbf{Demonstrations} & Demonstrations from different sets with reasoning (COT). \\
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{A broad structure of the prompt used for fine-tuning LLMs. }
\vspace{-1.75em}
\label{prompt-template}
\end{table}


==> tables/table-roberta-baseline.tex <==
\begin{table}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{3pt} % Adjust the spacing between columns
    \scalebox{0.85}{
    \begin{tabular}{@{}ccc|ccccc@{}}
    \hline
    \multicolumn{3}{c}{\textbf{Original Sets}} & \multicolumn{5}{c}{\textbf{Perturbed Sets}} \\
    \hline
    $\boldsymbol{\alpha_1}$ & $\boldsymbol{\alpha_2}$ & $\boldsymbol{\alpha_3}$ & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} \\
    \hline
    72.72 & 64.83 & 62.33 & 57.30 & 46.90 & 67.20 & 70.20 & 67.10 \\
    \hline
    \end{tabular}}
    \caption{\textbf{Baseline accuracy:} \model performance without any finetuning on perturbation sets.}
    \label{table-roberta-baseline}
\end{table}



==> tables/table-roberta-mixt.tex <==
\begin{table}[!ht]
\vspace{-0.5em}
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{2.75pt} % Adjust the spacing between columns
\scalebox{0.84}{
\begin{tabular}{@{}l|ccc|lllll|c@{}}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Original Sets}} & \multicolumn{5}{c}{\textbf{Challenge Sets}} & \multicolumn{1}{c}{} \\
\hline
$\boldsymbol{k}$ & $\boldsymbol{\alpha_1}$ & $\boldsymbol{\alpha_2}$ & $\boldsymbol{\alpha_3}$ & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & $\boldsymbol{\mu}$ \\
\hline
baseline &\bf 72.72 &  64.83 &  \bf 62.33 & \bf 57.30 & 46.90 & 67.20 & 70.20 & \bf 67.10 & - \\
\hline
100 & 70.40 & \bf 65.16 & 59.48 & 56.00 & 58.48 & 78.78 & 78.50 & 66.04 & 5.82 \\
200 & 70.42 & 65.06 & 59.21 & 56.86 & 59.50 & 80.94 & 80.36 & 64.68 & 6.73 \\
300 & 71.92 & 64.54 & 59.49 & 56.50 & 61.30 & 81.22 & 79.68 & 65.12 & 7.02 \\
400 & 72.11 & 64.48 & 59.78 & 56.58 & 63.70 & 81.60 & 80.38 & 64.64 & 7.64 \\
500 & 72.62 & 64.34 & 59.20 & 56.98 & \bf 66.06 & \bf 82.02 & \bf 80.52 & 65.64 & \textbf{8.50} \\
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{\textbf{\textsc{Mix}} \textbf{ Results :} \model finetuned on a mixed set of samples from different perturbation sets {\sc P}$_i$.}
\label{table-roberta-mixt}
\vspace{-1.5em}
\end{table}

==> tables/table-roberta-seq.tex <==
\begin{table}[!ht]
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{2pt} % Adjust the spacing between columns
\scalebox{0.85}{
\begin{tabular}{@{}l|lll|lllll|l@{}}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Original Test Sets}} & \multicolumn{5}{c}{\textbf{Challenge Test Sets} }\\
\hline
\textbf{Type} & $\boldsymbol{\alpha_1}$ & $\boldsymbol{\alpha_2}$ & $\boldsymbol{\alpha_3}$ & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan}& $\boldsymbol{\mu}$ \\
\hline
baseline &72.72 & \bf 64.83 & \bf 62.33 &  \bf 57.30 & 46.90 & 67.20 & 70.20 & 67.10 &  \\
\hline
\textbf{COL-ASC} & 61.67 & 60.94 & 50.11 & 48.80 & 54.60 & \bf 85.40 & 85.40 & 56.60 & \bf 4.42 \\
\textbf{COL-DSC} & \bf 74.67 & 62.72 & 60.44 & 58.90 & \bf 57.30 & 56.10 & 65.30 & \bf 68.00 & -0.62 \\
\textbf{ROW-ASC} & 55.00 & 58.11 & 47.22 & 46.80 & 50.90 & 84.50 & \bf 85.90 & 51.30 & 2.14\\
\textbf{ROW-DSC} & 73.44 & 63.39 & 57.44 & 56.50 & 45.10 & 60.00 & 71.60 & 65.80 & -1.94\\
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{\textbf{\textsc{Seq}}\textbf{ Results:} \model Sequential Training {\sc Seq} with 500 samples from each {\sc P$_k$}. Here, 
\textbf{{\sc col-asc: csnlm}}, \textbf{{\sc col-dsc: mlnsc}}, \textbf{{\sc row-asc: scnml}}, \textbf{{\sc row-dsc: lmncs}}. $\mu$ is the average improvement over baseline.}
\vspace{-0.75em}
\label{table-roberta-seq}
\end{table}

==> tables/table-roberta-varymix.tex <==
\begin{table}[!htb]
\vspace{-0.5em}
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{2.1pt} % Adjust the spacing between columns
\scalebox{0.875}{
\begin{tabular}{@{}l|ccc|ccccc|c@{}}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Original Sets}} & \multicolumn{5}{c}{\textbf{Challenge Sets}} & \multicolumn{1}{c}{} \\
\hline
$\boldsymbol{K}$ & $\boldsymbol{\alpha_1}$ & $\boldsymbol{\alpha_2}$ & $\boldsymbol{\alpha_3}$ & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & $\boldsymbol{\mu}$ \\
\hline
baseline & \bf 72.72 & \bf 64.83 & \bf 62.33 & \bf 57.30 & 46.90 & 67.20 & 70.20 & \bf 67.10 & - \\
\hline
500 & 71.28 & 64.42 & 60.39 & 56.26 & 59.22 & 77.84 & 76.24 & 65.38 & 5.25 \\
1000 & 71.07 & 64.72 & 59.60 & 57.04 & 63.24 & 79.94 & 79.06 & 65.50 & 7.22 \\
1500 & 72.07 & 64.81 & 59.73 & 56.50 & \bf 65.42 & \bf 80.84 & \bf 79.54 & 65.64 & \bf 7.85 \\
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{\textbf{\textsc{DynMix }}\textbf{Results:} \model fine tuned on $\boldsymbol{K}$ samples taken from all perturbation sets in ratio $0.201:0.245:0.182:0.200:0.172$ for $C:N:M:L:S$.}
\vspace{-1.0em}
\label{table-roberta-varymix}
\end{table}

==> tables/table-unpcot.tex <==
%\begin{table}[!ht]
%\vspace{-0.5em}
%\renewcommand{\arraystretch}{1.1}
%\centering
%\small
%\setlength{\tabcolsep}{3pt} % Adjust the spacing between columns
%\scalebox{0.85}{
%\begin{tabular}{p{0.7cm}|c|ccccccc}
%\hline
%Type &\textbf{Model} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & $R'$ \\
%\hline
%\multirow{3}{=}{\begin{sideways}\textbf{BASE}\end{sideways}} & LLaMA-2-70b  & 54.00 & 51.60 & 49.60 & 57.00 & 54.30 & 62.84 \\
%& LLaMA-2-13b & 39.67 & 39.33 & 45.67 & 56.67 & 44.67 & 45.20\\
%& GPT-3.5 & 51.00 & 53.00 & 62.66 & 61.00 & 60.30 & 69.45 \\
%\hline
%\multirow{3}{=}{\begin{sideways}\textbf{\textsc{OP$_{\text{CoT}}$}}\end{sideways}} %& LLaMA-2-70b & 63.00 & 60.00 & 63.00 & 61.30 & 66.00 &  70.82 \\ 
%& LLaMA-2-13b & 61.33 & 57.00 & 57.67 & 59.33 & 60.00 & 64.27\\
%& GPT-3.5 & 63.00 & 69.60 & 59.30 & 61.00 & 68.00 &  72.18\\ 
%\hline
%\end{tabular}}
%\vspace{-0.5em}
%\caption{\textbf{Few-shot with CoT ({\sc OP$_{\text{CoT}}$}).} Results using CoT prompting with exemplars sampled from {\sc O.}} 
%\label{table-unpcot}
%\vspace{-0.5em}
%\end{table}
% 63.00%	69.60%	59.30%	61.00%	68.00%  72.18%
% 61.33%	57.00%	57.67%	59.33%	60.00%	64.27%

\begin{table}[!ht]
\vspace{-0.5em}
\renewcommand{\arraystretch}{1.1}
\centering
\small
\setlength{\tabcolsep}{6pt} % Adjust the spacing between columns
\scalebox{0.80}{
\begin{tabular}{l|cccccc|cccccccc}
&  \multicolumn{6}{c|}{\bf BASE } &  \multicolumn{6}{c}{\bf \textbf{\textsc{OP$_{\text{CoT}}$}}} \\

\hline
\textbf{Model} & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & $R'$ & \textbf{char} & \textbf{neg} & \textbf{num} & \textbf{loc} & \textbf{stan} & $R'$ \\
\hline
LLaMA-2-70b  & 54.00 & 51.60 & 49.60 & 57.00 & 54.30 & 62.84 & 63.00 & 60.00 & 63.00 & 61.30 & 66.00 &  70.82 \\
LLaMA-2-13b & 39.67 & 39.33 & 45.67 & 56.67 & 44.67 & 45.20 & 61.33 & 57.00 & 57.67 & 59.33 & 60.00 & 64.27 \\
GPT-3.5 & 51.00 & 53.00 & 62.66 & 61.00 & 60.30 & 69.45  & 63.00 & 69.60 & 59.30 & 61.00 & 68.00 &  72.18 \\
%& LLaMA-2-70b & 63.00 & 60.00 & 63.00 & 61.30 & 66.00 &  70.82 \\ 
%& LLaMA-2-13b & 61.33 & 57.00 & 57.67 & 59.33 & 60.00 & 64.27\\
%& GPT-3.5 & 63.00 & 69.60 & 59.30 & 61.00 & 68.00 &  72.18\\ 
\hline
\end{tabular}}
\vspace{-0.5em}
\caption{\textbf{Few-shot with CoT ({\sc OP$_{\text{CoT}}$}).} Results using CoT prompting with exemplars sampled from {\sc O.}} 
\label{table-unpcot}
\vspace{-0.5em}
\end{table}


